Geometric Structure Aided Visual Inertial Localization

Visual Localization is an essential component in autonomous navigation. Existing approaches are either based on the visual structure from SLAM/SfM or the geometric structure from dense mapping. To take the advantages of both, in this work, we present a complete visual inertial localization system based on a hybrid map representation to reduce the computational cost and increase the positioning accuracy. Specially, we propose two modules for data association and batch optimization, respectively. To this end, we develop an efficient data association module to associate map components with local features, which takes only $2$ms to generate temporal landmarks. For batch optimization, instead of using visual factors, we develop a module to estimate a pose prior from the instant localization results to constrain poses. The experimental results on the EuRoC MAV dataset demonstrate a competitive performance compared to the state of the arts. Specially, our system achieves an average position error in 1.7 cm with 100% recall. The timings show that the proposed modules reduce the computational cost by 20-30%. We will make our implementation open source at http://github.com/hyhuang1995/gmmloc.

==> conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}

% STEP. long
% In this paper, we presented a monocular VO system leveraging deep description and repeatability.
% % We discuss
% % Different from previous work, we focus on explore a better way to.
% Not only extract the local features from the predicted repeatability, we further parameterize them as 2-D Gaussian component to model the uncertainty of prediction.
% Then, we propose a direct tracking scheme to estimate the camera pose coarsely.
% Afterwards, patch-wise association can be performed efficiently by check the inliers with neibourhoods.
% % To generate correspondences for triangualtion
% The experimetal results demonstrate the proposed system is capable to handle challenging situation, where both the state-of-the-art indirect and direct methods suffer from strong degradation.
% For the rumtime analysis, as the proposed system maintain a more lightweight backend than ORB-SLAM, the computation time of typical modules is dramatically reduced despite the feature extraction frontend.
% In the future, we would like to investigate supervising the feature detection and description frontend in an end-to-end manner.
% Introducing geometric constraints might benefits the learning process.

% STEP. short 
% TODO: rewrite
In this paper, we presented a monocular VO system leveraging learned description and repeatability.
% We discuss
Different from previous work, we focused on tightly coupling the learning-based frontend with indirect multiview geometry to fully exploit the network predictions.
% To achieve this goal, 
% the parameterization of local feature is discussed
% Not only extract the local features from the predicted repeatability, we further parameterize them as 2-D Gaussian component to model the uncertainty of prediction.
% To achieve this goal, we first extract local salient point
We proposed a two-step tracking scheme to estimate the camera pose: direct tracking on the repeatability maps and refining the pose with the patch-wise association.
The adapted mapping module maintained a lightweight and consistent backend.
% ANN along with grid-search on epipolar line associated features for triangualtion, with which a lightweight and consistent backend was maintained.
% Epipolar line search 
% Adapted mapping module 
% For the consideration of unc
% Adapted mapping module 
% The local feature parameterization was discussed to model the uncertainty.
% Grid search along epipolar line 
% Different mapping methods were discussed and adopted into the systematic implementation.
% Local feature parameterization 
%  coarsely.
% Afterwards, patch-wise association can be performed efficiently by check the inliers with neibourhoods.
% To generate correspondences for triangualtion
The experimental results demonstrated that the proposed system is capable to handle challenging situations, where both the state-of-the-art indirect and direct methods suffer from strong degradation.
% For the runtime analysis, as the proposed system maintain a more lightweight backend than ORB-SLAM, the computation time of typical modules is dramatically reduced despite the feature extraction frontend.
In the future, we would like to investigate supervising the feature detection and description frontend in an end-to-end manner and improving the network prediction speed for onboard visual state estimation.

    



==> section.tex <==
% \section{INTRODUCTION}
% \label{sec:intro}



% \cite{jeong2017road}


% \section{States, Residuals and Jacobians}
\subsection{State Definition, Update and Prediction}
We first recap the state definitions.
As in the paper, the state vector for $k$-th frame is defined by:
\begin{equation}
	\mathbf{x}_k = \left[
	\boldsymbol{\phi}_k,
	\mathbf{t}_k,
	\mathbf{v}_k,
	% \mathbf{R}_{B_kW},
	% {^{B_k}\mathbf{t}_{B_kW}},
	% {^W\mathbf{v}_{B_k}},
	{\mathbf{b}^g_{k}},
	{\mathbf{b}^a_{k}
	}
	\right]
\end{equation}
where the rotation and translation of the body frame are:
\begin{equation}
	\mathbf{R}_{B_kW} = \exp({\boldsymbol{\phi}_k}^\land), \quad
	{^{B_k}\mathbf{t}_{B_kW}} = \mathbf{t}_k
\end{equation}
% where the states have the same definitions in the original paper.
In our implementation, the update of states is defined by:
\begin{equation}
	\mathbf{x}_k \leftarrow \mathbf{x}_k \boxplus \delta \mathbf{x}_k =
	\left[
		\begin{matrix}
			\exp({\boldsymbol{\phi}_k}^\land)\exp({\delta \boldsymbol{\phi}_k}^\land) \\
			\mathbf{t}_k + \delta \mathbf{t}_k                                        \\
			\mathbf{v}_k + \delta \mathbf{v}_k                                        \\
			\mathbf{b}_k^g + \delta \mathbf{b}_k^g                                    \\
			\mathbf{b}_k^a + \delta \mathbf{b}_k^a
		\end{matrix}
		\right]
\end{equation}

% \subsection{State Prediction}
% With inertial measurement, the state of 
We apply the method proposed in \cite{forster2016manifold} to convert raw inertial measurements into pre-integrated factors $\Delta \mathbf{R}_{kk+1}$, $\Delta \mathbf{v}_{kk+1}$ and $\Delta \mathbf{t}_{kk+1}$.
With inertial pre-integration, the camera pose of incoming frame $\mathbf{R}_{WB_{k+1}}, {^W\mathbf{t}_{B_{k+1}}}$can be predicted by:
\begin{equation}
	\begin{aligned}
		\mathbf{R}_{WB_{k+1}}    & = \mathbf{R}_{WB_{k}}\Delta \mathbf{R}_{{k} {k+1}} \exp(\mathbf{J}_{\Delta R}^g \delta \mathbf{b}^g_k),                                                  \\
		% \mathbf{R}_{WB_{k+1}} &= \mathbf{R}_{WB_{k}}\Delta \mathbf{R}_{B_{k} B_{k+1}} \exp(\mathbf{J}_{\Delta R}^g \mathbf{b}_g^k)\\
		{^W\mathbf{v}_{B_{k+1}}} & = {^W\mathbf{v}}_{B_{k}}+\mathbf{g}_{W} \Delta t_{k}                                                                                                 \\
		                         & + \mathbf{R}_{WB_k}\left(\Delta \mathbf{v}_{k k+1}+\mathbf{J}_{\Delta v}^{g} \delta \mathbf{b}^{g}_{k}+\mathbf{J}_{\Delta v}^{a} \delta \mathbf{b}^{a}_{k}\right), \\
		{^W\mathbf{t}}_{B_{k+1}} & = {^W\mathbf{t}_{B_k}} + {^{W}\mathbf{v}_{B_k}} \Delta t_{k}+\frac{1}{2} {^W\mathbf{g}} \Delta t_{k}^{2}                                             \\
		                         & +\mathbf{R}_{WB_k}\left(\Delta \mathbf{t}_{k k+1}+\mathbf{J}_{\Delta p}^{g} \delta \mathbf{b}^{g}_{k}+\mathbf{J}_{\Delta p}^{a} \delta \mathbf{b}^{a}_{k}\right),
	\end{aligned}
\end{equation}
where 
$\mathbf{J}^g_{\Delta R}$
$\mathbf{J}^g_{\Delta v}$
$\mathbf{J}^a_{\Delta v}$
$\mathbf{J}^g_{\Delta t}$
$\mathbf{J}^a_{\Delta t}$ are the jacobians of pre-integrated terms w.r.t the bias update $\mathbf{b}_k^g$ and $\mathbf{b}_k^a$.
For vision-only system, we apply constant-velocity model to predict the current pose:
\begin{equation}
	\begin{aligned}
		\mathbf{R}_{WB_{k+1}} = \mathbf{R}_{WB_{k}} (\mathbf{R}_{B_{k-1}W}\mathbf{R}_{WB_k}) \\
		^W\mathbf{t}_{WB_{k+1}} =
		2{^W\mathbf{t}_{WB_{k}}} - {^W\mathbf{t}_{WB_{k-1}}}
	\end{aligned}
\end{equation}

\subsection{Residual Definition and Jacobians}

The residual terms used in the implementation are defined as follows:
for the visual factors, we define the residual as the reprojection error:
\begin{equation}
	\mathbf{e}_\text{proj} = \pi({^{C_k}\mathbf{p}_i}) - \bar{\mathbf{u}}_{ik},
\end{equation}
\begin{equation}
	^{C_k}\mathbf{p}_i = \mathbf{R}_{CB} (\mathbf{R}_{B_kW} {^
	W\mathbf{p}_i}+ {^{B_k}\mathbf{t}_{B_kW}}) + {^{C}\mathbf{t}_{CB}},
\end{equation}
where ${^{C_k}\mathbf{p}_i}$ is the landmark position under frame $C_k$.
$\bar{\mathbf{u}}_{ik}$ is the local observation for ${^W}\mathbf{p}_i$.

The inertial residual is defined by:
\begin{equation}
	\mathbf{e}_\text{inertial} = \left[\mathbf{e}_\text{rot}^T, \mathbf{e}_\text{pos}^T, \mathbf{e}_\text{vel}^T, \mathbf{e}_\text{bias}^T\right]^T ,
\end{equation}
where we have
\begin{equation}
	\begin{aligned}
		\mathbf{e}_{\text{rot}}  & = \log\left(\left(\Delta\mathbf{R}_{kj}\exp(\mathbf{J}_{\Delta R}^g \mathbf{b}_g^j)\right)\mathbf{R}_{B_{k}W}\mathbf{R}_{WB_{j}}\right) ^ \lor ,                                       \\
		\mathbf{e}_{\text{vel}}  & =\mathbf{R}_{B_{j}W} \Delta \mathbf{v}_{jk} -\left({\Delta \tilde{\mathbf{v}}_{jk}}+\mathbf{J}_{\Delta v}^{g} \delta \mathbf{b}_{g}^{j}+\mathbf{J}_{\Delta v}^{a} \delta \mathbf{b}_{a}^{j}\right) , \\
		\mathbf{e}_{\text{pos}}  & =\mathbf{R}_{B_{j}W}
		\Delta \mathbf{t}_{jk} -\left(\Delta \tilde{\mathbf{t}}_{jk}+\mathbf{J}_{\Delta t}^{g} \delta \mathbf{b}_{g}^{j}+\mathbf{J}_{\Delta t}^{a} \delta \mathbf{b}_{a}^{j}\right) ,                                                   \\
		\mathbf{e}_{\text{bias}} & =\mathbf{b}^{j}-\mathbf{b}^{k} ,
	\end{aligned}
\end{equation}
with $\Delta \mathbf{v}_{jk}$ and $\Delta \mathbf{t}_{jk}$ given by:
\begin{equation}
	\Delta \mathbf{v}_{jk} = {^{W} \mathbf{v}_{B_k}} - {^{W} \mathbf{v}_{B_j}} -{^{W}\mathbf{g}} \Delta t_{jk}
\end{equation}
\begin{equation}
	\Delta \mathbf{t}_{jk} =  {^W\mathbf{t}_{B_k}}- {^{W} \mathbf{t}_{B_j}} - {^W\mathbf{v}_{B_j}} \Delta t_{jk} - \frac{1}{2} {^W\mathbf{g}} \Delta t_{jk}^{2}
\end{equation}
where $\Delta \tilde{\mathbf{R}}_{kj}, \Delta \tilde{\mathbf{v}}_{kj}, \Delta \tilde{\mathbf{t}}_{kj}$ are from the pre-integration,
$\mathbf{J}^g_{\Delta R}$
$\mathbf{J}^g_{\Delta v}$
$\mathbf{J}^a_{\Delta v}$
$\mathbf{J}^g_{\Delta t}$
$\mathbf{J}^a_{\Delta t}$ are the jacobians related to bias update.
This formulation is similar to \cite{forster2016manifold, mur2017visual}.

The jacobians of different residual terms w.r.t different states are derived as:
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{proj}}{\partial \delta \mathbf{x}_k} =
	\frac{\partial \mathbf{e}_\text{proj}}{\partial {^{C_k}\mathbf{p}_i}} \cdot
	\frac{\partial {^{C_k}\mathbf{p}_i}}{\partial \delta \mathbf{x}_k}
	% \frac{}{}
\end{equation*}
\begin{equation*}
	\frac{\partial {^{C_k}\mathbf{p}_i}}{\partial \delta \boldsymbol{\phi}_k} =
	-\mathbf{R}_{CB}\mathbf{R}_{BW} \cdot {^W\mathbf{p}_i}^\land ,
	\quad
	\frac{\partial {^{C_k}\mathbf{p}_i}}{\partial \delta \mathbf{t}_k} =
	\mathbf{R}_{CB},
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{rot}}{\partial \delta \boldsymbol{\phi}_k}	= \mathbf{J}_{r}^{-1}\left({\mathbf{e}_\text{rot}} \right) \mathbf{R}_{B_kW}, \quad
	\frac{\partial \mathbf{e}_\text{rot}}{\partial \delta \boldsymbol{\phi}_j}	= -\mathbf{J}_{r}^{-1}\left( \mathbf{e}_\text{rot} \right) \mathbf{R}_{B_jW},
\end{equation*}

\begin{equation*}
	\frac{\partial \mathbf{e}_\text{rot}}{\partial \delta \boldsymbol{\phi}_k}	= \mathbf{J}_{r}^{-1}\left({\mathbf{e}_\text{rot}} \right) \mathbf{R}_{B_kW}, \quad
	\frac{\partial \mathbf{e}_\text{rot}}{\partial \delta \boldsymbol{\phi}_j}	= -\mathbf{J}_{r}^{-1}\left( \mathbf{e}_\text{rot} \right) \mathbf{R}_{B_jW},
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{rot}}{\partial \delta \mathbf{b}_g^j}	= \mathbf{J}_{r}^{-1} \cdot \left( \mathbf{e}_\text{rot} \right) \mathbf{R}_{B_jW} \mathbf{R}_{WB_k} \cdot \mathbf{J}_r \left(\mathbf{J}^g_{\Delta R} \mathbf{b}_g^j\right),
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{vel}}{\partial \delta\boldsymbol{\phi}_j} = -\mathbf{R}_{B_jW} \cdot {\Delta \mathbf{v}_{jk}}^\land, \quad
	\frac{\partial \mathbf{e}_\text{vel}}{\partial \delta\mathbf{v}_j} = \mathbf{R}_{B_jW},
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{vel}}{\partial \delta\mathbf{v}_k} = -\mathbf{R}_{B_jW}, \quad
	\frac{\partial \mathbf{e}_\text{vel}}{\partial \delta\mathbf{b}^j_g} = -\mathbf{J}_{\Delta v}^g , \quad
	\frac{\partial \mathbf{e}_\text{vel}}{\partial \delta\mathbf{b}^j_a} = -\mathbf{J}_{\Delta v}^a,
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\boldsymbol{\phi}_j} = -\mathbf{R}_{B_jW} \cdot {\Delta \mathbf{t}_{jk}}^\land , \quad
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\boldsymbol{\phi}_k} = \mathbf{R}_{B_jW} \cdot {\mathbf{t}_{WB_k}}^\land,
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\mathbf{t}_k} = -\mathbf{R}_{B_jW} \mathbf{R}_{B_kW}^T , \quad
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\mathbf{t}_j} = \mathbf{I}_{3 \times 3} ,
	%  \mathbf{R}_{B_jW} \Delta t_{jk} 
\end{equation*}
\begin{equation*}
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\mathbf{v}_j} =
	- \mathbf{R}_{B_jW} \Delta t_{jk} , \quad
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\mathbf{b}^j_g} =
	- \mathbf{J}^g_{\Delta t} , \quad
	\frac{\partial \mathbf{e}_\text{pos}}{\partial \delta\mathbf{b}^j_a} =
	- \mathbf{J}^a_{\Delta t} .
\end{equation*}

\begin{figure*}[t!]
	\centering
	\includegraphics[width=1.0\textwidth]{fig/v103_cov_ill.pdf}\\
	\includegraphics[width=1.0\textwidth]{fig/v201_cov_ill.pdf}
	\caption{The trace of covariance and Absolute Pose Error (APE) on V103 (top) and V201 (bottom), along with some excerpts that show local features matched with landmarks in both temporal (shown in red) and prior (shown in blue) structures.}
	\label{fig.ratio_loc_err}
\end{figure*}
\subsection{Covariance Recovery}
\subsubsection{Explanation}
In the manuscript, we provide a general description for covariance recovery,
here we give a more detailed explanation along with some example results.
Assuming that we would like to recover the covariance of $^W\mathbf{t}_{WB_k}$.
In the instant localization, we estimate relevant states via the following optimization problem:
\begin{equation*}
	\begin{aligned}
	\hat{\mathbf{x}}_k, \hat{\mathbf{x}}_{k - 1} = {\arg \min}_{\mathbf{x}_k, \mathbf{x}_{k-1}} &E_\text{inertial}(\mathbf{x}_k, \mathbf{x}_{k-1}) + E_\text{prior}(\mathbf{x}_k) \\
	&+ \sum_{i \in \mathcal{V}_k} E_\text{proj}(\boldsymbol{\xi}_k, {^W\mathbf{p}_i}),
	\end{aligned}
\end{equation*}
which resulting in solving the following normal equation:
\begin{equation}
	\mathbf{H} \delta \mathbf{x} = \mathbf{b},
\end{equation}
where $\mathbf{H}$ and $\mathbf{b}$ are the information matrix and vector, $\delta \mathbf{x}$ is the update of the state vector, respectively.
To recover the covariance of $^W\mathbf{t}_{WB_k}$, we first reorder the state vector as $[\mathbf{t}_k, \mathbf{x}_{r}]$,
$\mathbf{x}_r$ is for the rest states, then we have:
\begin{equation}
	\left[
		\begin{matrix}
			\mathbf{H}_{tt} & \mathbf{H}_{tr} \\
			\mathbf{H}_{rt} & \mathbf{H}_{rr} \\
		\end{matrix}
		\right]
	\left[
		\begin{matrix}
			\delta \mathbf{t}_k \\
			\delta \mathbf{x}_r \\
		\end{matrix}
		\right]
	=
	\left[
		\begin{matrix}
			\mathbf{b}_t \\
			\mathbf{b}_r \\
		\end{matrix}
		\right].
\end{equation}
By applying schur complement, we have
\begin{equation}
	\label{eq.normal_schur}
	\bar{\mathbf{H}}_{tt} \delta \mathbf{t}_k = \bar{\mathbf{b}}_{t},
\end{equation}
with
\begin{equation}
	\bar{\mathbf{H}}_{tt} = \mathbf{H}_{tt} - \mathbf{H}_{tr}\mathbf{H}_{rr}^{-1}\mathbf{H}_{rt}, \quad
	\bar{\mathbf{b}}_{t} = \mathbf{b}_{t} - \mathbf{H}_{tr} \mathbf{H}_{rr}^{-1} \mathbf{b}_r.
\end{equation}
With \textit{Proposition. 1} and \textit{Proposition. 2}, \autoref{eq.normal_schur} forms a prior distribution on $\delta \mathbf{t}_k$, $\delta \mathbf{t}_k \sim \mathcal{N}(\delta \hat{\mathbf{t}}_k, \boldsymbol{\Sigma}_{tt})$, with $\boldsymbol{\Sigma}_{tt} = \bar{\mathbf{H}}_{tt}^{-1}$.
To obtain the covariance of translation under map frame, i.e., $^W\mathbf{t}_{WB_k}$, we can simply propagate the covariance via:
\begin{equation}
	\boldsymbol{\Sigma}_{t} = \mathbf{R}_{WB} \boldsymbol{\Sigma}_{tt}\mathbf{R}_{BW}
\end{equation}

\textit{Proposition 1.} With the measurement noise modelled by Gaussian,
in a least-squares problem, the covariance of states can be approximated by $\boldsymbol{\Sigma} = \mathbf{H}^{-1}$ when reaching optimal.

\textit{Proof 1.}
Given the measurement function as:
\begin{equation}
	\mathbf{z} = h\left(\mathbf{x}\right) + \mathbf{n}_z, \quad \mathbf{n}_z \sim \mathcal{N}(\mathbf{0}, \boldsymbol{\Sigma}_z).
\end{equation}
When the estimation reaching the optimal, we can linearize it as:
\begin{equation}
	\mathbf{z} = h\left(\hat{\mathbf{x}}\right) + \mathbf{J}\delta \mathbf{x}, \quad \text{with} \quad
	\mathbf{J} = \frac{\partial h(\hat{\mathbf{x}} \boxplus \delta \mathbf{x})}{\partial \delta \mathbf{x}}.
\end{equation}
By propagating the uncertainty, we have:
\begin{equation}
	\boldsymbol{\Sigma}_z = \mathbf{J} \boldsymbol{\Sigma} \mathbf{J}^T.
\end{equation}
Apply inversion on both side, we have:
\begin{equation}
	\boldsymbol{\Sigma}_z^{-1} = \left(\mathbf{J} \boldsymbol{\Sigma} \mathbf{J}^T\right)^{-1},
\end{equation}
thus we have $\boldsymbol{\Sigma} = \left(\mathbf{J}^T\boldsymbol{\Sigma}_z^{-1}\mathbf{J}\right)^{-1} = \mathbf{H}^{-1}$.


\textit{Proposition 2.} 
By applying Schur Complement to recover state covariance, the above scheme forms a marginal distribution, given as:
\begin{equation*}
p\left(\delta \mathbf{t}_{k} \mid \mathbf{z}_{rt}\right)=\int_{\delta \mathbf{x}_{r}} p\left(\delta \mathbf{t}_{k}, \delta \mathbf{x}_{r} \mid \mathbf{z}_{rt}\right) d \delta \mathbf{x}_{r} \approx \mathcal{N}\left(\delta\hat{\mathbf{t}}_{k}, \boldsymbol{\Sigma}_{tt}\right)
\end{equation*}
where the joint distribution of $\left[\delta \mathbf{t}_{k}^T, \delta \mathbf{x}_{r}^T\right]^T$ is given by:
\begin{equation*}
	\left[
		\begin{matrix}
			\delta \mathbf{t}_{k}  \\
			\delta \mathbf{x}_{r}  \\
		\end{matrix}
	\right]
	\sim \mathcal{N} \left(
	\left[
		\begin{matrix}
			\delta \mathbf{t}_{k}  \\
			\delta \mathbf{x}_{r}  \\
		\end{matrix}
	\right],
	\left[
		\begin{matrix}
			\boldsymbol{\Sigma}_{tt} & \boldsymbol{\Sigma}_{tr} \\
			\boldsymbol{\Sigma}_{rt} & \boldsymbol{\Sigma}_{rr} \\
		\end{matrix}
	\right]
	\right)
\end{equation*}

\textit{Proof 2.} 
By applying the \textit{Woodbury-formula}, with \textit{Proposition 1.}, we have the inverse of Covariance:
\begin{equation*}
	\begin{aligned}
	&\boldsymbol{\Sigma} = 
	\left[
		\begin{matrix}
			\boldsymbol{\Sigma}_{tt} & \boldsymbol{\Sigma}_{tr} \\
			\boldsymbol{\Sigma}_{rt} & \boldsymbol{\Sigma}_{rr} \\
		\end{matrix}
	\right]
	=
	\left[
		\begin{matrix}
			\mathbf{H}_{tt} & \mathbf{H}_{tr} \\
			\mathbf{H}_{rt} & \mathbf{H}_{rr} \\
		\end{matrix}
	\right]^{-1} = \\
	&\left[
		\begin{matrix}
			\mathbf{1} & \mathbf{H}_{tr} \mathbf{H}_{rr}^{-1} \\
			\mathbf{0} & \mathbf{1} \\
		\end{matrix}
	\right]
	\left[
		\begin{matrix}
			\mathbf{H}_{tt} + \mathbf{H}_{tr}\mathbf{H}_{rr}^{-1}\mathbf{H}_{rt} & \mathbf{0} \\
			\mathbf{0} & \mathbf{H}_{rr} \\
		\end{matrix}
	\right]
	\left[
		\begin{matrix}
			\mathbf{1} & \mathbf{0} \\
			\mathbf{H}_{rr}^{-1}\mathbf{H}_{rt} & \mathbf{1} \\
		\end{matrix}
	\right]
	\end{aligned}
\end{equation*}.
Therefore we have $\boldsymbol{\Sigma}_{tt} = \mathbf{H}_{tt} - \mathbf{H}_{tr}\mathbf{H}_{rr}^{-1}\mathbf{H}_{rt} = \bar{\mathbf{H}}_{tt}^{-1}$, which has exactly the same form with the Covariance derived above.

\subsubsection{Experimental Results}
We provide some experimental results to further show the uncertainty estimation, shown in \autoref{fig.ratio_loc_err}.
Generally, the localization error is coherent with the magnitude of covariance corresponding to the translational part.
Another interesting observation is that, according to the excerpts, when total number of matched features or matched prior landmarks is insufficient, the uncertainty of estimation tends to be large.


\subsection{Detailed Timing Results}

We report the detailed timing results in \autoref{tab.timing}, where the timing results of Pred and Opt correspond to the results in the manuscript.
% Timing result
In general, Ours(V+I+L) achieves a real time performance in single thread (28.8 ms on V201 and 38.0ms on V103), while Ours(V+P) can be a little bit time-consuming (37.4 ms on V201 and 54.9 ms on V103).
\begin{table}[tbp]
	\caption{Runtime comparison on V201 (top) and V103 (bottom) for different modules: Re-localization (Re-Loc), global feature extraction (Feat(G)), local feature extraction (Feat(L)), State Prediction (Pred), instant localization (Track), temporal landmark verification (Update), temporal landmark generation (Creation) and windowed optimization (Opt). Modules marked with (*) are only called when necessary.
		The proposed association step and optimization strategy do improve the efficiency of the complete system.
	}
	\label{tab.timing}
	\centering
	\begin{tabular}{lcccc}
		\toprule
		\textbf{Modules} & \textbf{Ours(V+P)}                    & \textbf{Ours(V)} & \textbf{Ours(V+I)} & \textbf{Ours(V+I+L)} \\ %\Tstrut{}
		\midrule
		Feat(G)*         & \multicolumn{4}{c}{ 29.1 $\pm$ 0.0 }                                                                 \\
		Re-Loc*          & \multicolumn{4}{c}{ 105.0 $\pm$ 0.0 }                                                                \\
		Feat(L)          & \multicolumn{4}{c}{ 17.7 $\pm$ 0.3 }                                                                 \\\midrule
		Pred             & 0.2 $\pm$ 0.0                         & 0.2 $\pm$ 0.0    & 0.2 $\pm$ 0.0      & 0.2 $\pm$ 0.0        \\
		Track            & 9.1 $\pm$ 0.2                         & 9.1 $\pm$ 0.2    & 8.7 $\pm$ 0.1      & 8.6 $\pm$ 0.1        \\
		Update           & 0.4 $\pm$ 0.0                         & 0.4 $\pm$ 0.0    & 0.4 $\pm$ 0.0      & 0.4 $\pm$ 0.0        \\\midrule
		Creation*        & 9.3 $\pm$ 9.6                         & 2.5 $\pm$ 0.9    & 2.4 $\pm$ 0.7      & 2.4 $\pm$ 0.7        \\
		Opt*             & 50.4 $\pm$ 22.1                       & 49.4 $\pm$ 24.2  & 23.4 $\pm$ 6.9     & 8.0 $\pm$ 1.9        \\ \midrule
		Total            & 37.4 $\pm$ 0.3                        & 36.2 $\pm$  0.2  & 31.4 $\pm$ 0.2     & 28.8 $\pm$ 0.1       \\ \bottomrule
	\end{tabular}

	\vspace{0.5em}
	\begin{tabular}{lcccc}
		\toprule
		\textbf{Modules} & \textbf{Ours(V+P)}                    & \textbf{Ours(V)} & \textbf{Ours(V+I)} & \textbf{Ours(V+I+L)} \\ %\Tstrut{}
		\midrule
		Feat(G)*         & \multicolumn{4}{c}{ 29.9 $\pm$ 0.0 }                                                                 \\
		Re-Loc*          & \multicolumn{4}{c}{ 141.6 $\pm$ 0.0 }                                                                \\
		Feat(L)          & \multicolumn{4}{c}{ 16.9 $\pm$ 0.6 }                                                                 \\\midrule
		Pred             & 0.1 $\pm$ 0.0                         & 0.1 $\pm$ 0.0    & 0.1 $\pm$ 0.0      & 0.1 $\pm$ 0.0        \\
		Track            & 15.7 $\pm$ 4.1                        & 15.9 $\pm$ 0.2   & 15.2 $\pm$ 0.1     & 15.0 $\pm$ 0.1       \\
		Update           & 0.5 $\pm$ 0.0                         & 0.4 $\pm$ 0.0    & 0.4 $\pm$ 0.0      & 0.4 $\pm$ 0.0        \\\midrule
		Creation*        & 4.9 $\pm$ 1.4                         & 1.2 $\pm$ 0.3    & 1.2 $\pm$ 0.3      & 1.2 $\pm$ 0.3        \\
		Opt*             & 38.6 $\pm$ 11.3                       & 33.3 $\pm$ 9.1   & 13.1 $\pm$ 4.0     & 4.8 $\pm$ 1.0        \\ \midrule
		Total            & 54.9 $\pm$ 5.1                        & 51.1 $\pm$ 0.3   & 41.6 $\pm$ 0.3     & 38.0 $\pm$ 0.3       \\ \bottomrule
	\end{tabular}

	\vspace{-1.5em}
\end{table}

==> timing.tex <==
\begin{table}[htbp]
    \centering
    \caption{Timing test for different modules.}
    \label{tab:timing}
    \begin{tabular}{ccccc}
        \hline
           Module  & \textbf{Mean (s)} & \textbf{Median (s)}  \\ \hline
        Tracking &  0.0287         & 0.0265                 \\
        Mapping & 0.0468         &  0.0445                \\ \hline
    \end{tabular}
\end{table}

\autoref{tab:timing} shows the timing results of tracking and mapping module. The processing frequency of tracking front-end is approximately 30Hz, which justifies the real-time performance of our system.
